Algebraic Quantum Intelligence: A New Framework for Reproducible Machine Creativity

Large language models (LLMs) have achieved remarkable success in generating fluent and contextually appropriate text; however, their capacity to produce genuinely creative outputs remains limited. This paper posits that this limitation arises from a structural property of contemporary LLMs: when provided with rich context, the space of future generations becomes strongly constrained, and the generation process is effectively governed by near-deterministic dynamics. Recent approaches such as test-time scaling and context adaptation improve performance but do not fundamentally alter this constraint. To address this issue, we propose Algebraic Quantum Intelligence (AQI) as a computational framework that enables systematic expansion of semantic space. AQI is formulated as a noncommutative algebraic structure inspired by quantum theory, allowing properties such as order dependence, interference, and uncertainty to be implemented in a controlled and designable manner. Semantic states are represented as vectors in a Hilbert space, and their evolution is governed by C-values computed from noncommutative operators, thereby ensuring the coexistence and expansion of multiple future semantic possibilities. In this study, we implement AQI by extending a transformer-based LLM with more than 600 specialized operators. We evaluate the resulting system on creative reasoning benchmarks spanning ten domains under an LLM-as-a-judge protocol. The results show that AQI consistently outperforms strong baseline models, yielding statistically significant improvements and reduced cross-domain variance. These findings demonstrate that noncommutative algebraic dynamics can serve as a practical and reproducible foundation for machine creativity. Notably, this architecture has already been deployed in real-world enterprise environments.

==> figures/fig5_6.tex <==
\begin{figure}[!tbp]
\centering
\begin{minipage}[t]{0.49\linewidth}
\centering
\includegraphics[
    width=\linewidth,
    trim=2.2cm 1.5cm 0cm 0cm,
    clip
]{fig-5}
\caption{Order-dependent semantic divergence induced by non-commutative operators. Embedding projections (PCA) of outputs generated under two conditions---\(A\to B\) (Super CFO \(\to\) Super CHRO) and \(B\to A\)---form clearly separated clusters even at temperature = 0, demonstrating systematic trajectory bifurcation driven solely by operator order.}
\label{fig:5}
\end{minipage}\hfill
\begin{minipage}[t]{0.49\linewidth}
\centering
\includegraphics[
    width=\linewidth,
    trim=3.7cm 2.5cm 0cm 0cm,
    clip
]{fig-6}
\caption{Evidence of interference effects in non-commutative semantic composition. Correlation analysis shows that changes in responses induced by sequential operator application cannot be explained by commutative linear composition, revealing interference-like modulation where semantic components are selectively amplified or suppressed.}
\label{fig:6}
\end{minipage}
\end{figure}


